Search for supersymmetry in events with $b$-tagged jets and missing transverse momentum in $pp$ collisions at $\sqrt{s}=13$ TeV with the ATLAS detector

A search for the supersymmetric partners of the Standard Model bottom and top quarks is presented. The search uses 36.1 fb$^{-1}$ of $pp$ collision data at $\sqrt{s}=13$ TeV collected by the ATLAS experiment at the Large Hadron Collider. Direct production of pairs of bottom and top squarks ($\tilde{b}_{1}$ and $\tilde{t}_{1}$) is searched for in final states with $b$-tagged jets and missing transverse momentum. Distinctive selections are defined with either no charged leptons (electrons or muons) in the final state, or one charged lepton. The zero-lepton selection targets models in which the $\tilde{b}_{1}$ is the lightest squark and decays via $\tilde{b}_{1} \rightarrow b \tilde{\chi}^{0}_{1}$, where $\tilde{\chi}^{0}_{1}$ is the lightest neutralino. The one-lepton final state targets models where bottom or top squarks are produced and can decay into multiple channels, $\tilde{b}_{1} \rightarrow b \tilde{\chi}^{0}_{1}$ and $\tilde{b}_{1} \rightarrow t \tilde{\chi}^{\pm}_{1}$, or $\tilde{t}_{1} \rightarrow t \tilde{\chi}^{0}_{1}$ and $\tilde{t}_{1} \rightarrow b \tilde{\chi}^{\pm}_{1}$, where $\tilde{\chi}^{\pm}_{1}$ is the lightest chargino and the mass difference $m_{\tilde{\chi}^{\pm}_{1}}- m_{\tilde{\chi}^{0}_{1}}$ is set to 1 GeV. No excess above the expected Standard Model background is observed. Exclusion limits at 95\% confidence level on the mass of third-generation squarks are derived in various supersymmetry-inspired simplified models.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Adjust TEXLIVE if it is not correct, or pass it to "make new".
# Replace BIBTEX = bibtex with BIBTEX = biber if you use biber instead of bibtex.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to rmeove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# If you have to run latex rather than pdflatex adjust the dependencies of %.dvi target
#   and use the command "make run_latex" to compile.
# Specify dvipdf or dvips as the run_latex dependency,
#   depending on which you want to use.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
# BIBTEX = biber
DVIPS    = dvips
DVIPDF   = dvipdf

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = SbottomPaper2017
#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figures
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with pdflatex
default: run_pdflatex

.PHONY: new newtexmf newbook newbooktexmf draftcover preprintcover auxmat \
	clean cleanpdf help

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf:	%.tex *.tex bibtex/bib/*.bib
%.pdf:	%.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

new:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document.tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document.tex >$(BASENAME).tex; \
	fi
	cp template/atlas-document-metadata.tex $(BASENAME)-metadata.tex
	touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newtexmf:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document-texmf.tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document-texmf.tex >$(BASENAME).tex; \
	fi
	cp template/atlas-document-metadata.tex $(BASENAME)-metadata.tex
	touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newbook:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-book.tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-book.tex >$(BASENAME).tex; \
	fi
	cp template/atlas-document-metadata.tex $(BASENAME)-metadata.tex
	touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newbooktexmf:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-book-texmf.tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-book-texmf.tex >$(BASENAME).tex; \
	fi
	cp template/atlas-document-metadata.tex $(BASENAME)-metadata.tex
	touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

draftcover:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-draft-cover.tex \
	    >$(BASENAME)-draft-cover.tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  cp  template/$(BASENAME)-draft-cover.tex $(BASENAME)-draft-cover.tex; \
	fi

preprintcover:
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-preprint-cover.tex >$(BASENAME)-preprint-cover.tex
	#cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

auxmat:
	sed s/atlas-document/$(BASENAME)/ template/atlas-auxmat.tex | \
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME)-auxmat.tex

run_latex: dvipdf

# Targets if you run latex instead of pdflatex
dvipdf:	$(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $(basename $<).pdf"

dvips:	$(BASENAME).dvi
	$(DVIPS) $<
	@echo "Made $(basename $<).ps"

# Specify dependencies for running latex
#%.dvi:	%.tex tex/*.tex bibtex/bib/*.bib
%.dvi:	%.tex *.tex *.bib
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $<
	$(BIBTEX) $<

help:
	@echo "To create a new document give the commands:"
	@echo "make new [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly." 
	@echo ""
	@echo "If you want to write a long document (book) like a TDR:"
	@echo "make newbook [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newtexmf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "make newbooktexmf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-preprint-cover"
	@echo ""
	@echo "If you need a document for auxiliary material give the commands:"
	@echo "make auxmat [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-auxmat"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanps  to clean output PS files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo ""

clean:
	-rm *.dvi *.toc *.aux *.log *.out \
		 *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx \
		*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf 
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-auxmat.pdf

cleanps:
	-rm $(BASENAME).ps 
	-rm $(BASENAME)-draft-cover.ps $(BASENAME)-preprint-cover.ps
	-rm $(BASENAME)-auxmat.ps

cleanall: clean cleanpdf cleanps

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^


==> journal/Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-elsevier atlas-jhep atlas-revtex

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf


==> journal/atlas-document-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%% Title
\AtlasTitle{A simple ATLAS paper draft}
%
% Author - this does not work with revtex
% \author{The ATLAS Collaboration}
%
% Date: if not given, uses current date
% \date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{1.0}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2014-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2014-XXX}
% \AtlasNote{ATLAS-PUB-2014-XXX}
\AtlasNote{ATLAS-COM-PHYS-2014-XXX}

% Submission journal
\AtlasJournal{Phys.\ Lett.\ B.}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
	This is a bare bones ATLAS document used to demonstrate how to use journal templates.

	This document is typeset using the \DocumentStyle.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% Explicit list of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{A supporting note}{http://cds.cern.ch/record/XXXXXX}
\AtlasCoverSupportingNote{Another supporting note}{http://cds.cern.ch/record/YYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{DD Month 2014}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
\AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-GROUP-2014-XX-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-GROUP-2014-XX-editorial-board@cern.ch}

% CERN preprintnumber
\PreprintIdNumber{CERN-PH-2014-XX}

